Cost-Aware Exploration for Chiplet-Based Architecture with Advanced Packaging Technologies

The chiplet-based System-in-Package~(SiP) technology enables more design flexibility via various inter-chiplet connection and heterogeneous integration. However, it is not known how to convert such flexibility into cost efficiency, which is critical when making a design decision. In this paper, we develop an analytical cost model that can estimate the cost of the 2.5D chiplet-based SiP systems under various interconnection options and technology nodes. We conducted two case studies using our cost model to explore the cost characteristics of the 2.5D chiplet-based SiP system. Based on the case studies, we made several observations on the interposer selection, design partition granularity, and technology node adoption for cost-efficient chiplet-based SiP design.

==> discussion.tex <==
% \section{Discussion}
% \label{sec:discussion}

% Besides the manufacture cost and the package cost discussed in this paper, the testing cost and the cooling cost also play an important role in the early-stage design decision.

% \subsection{Testing Cost Model}
% \subsection{Cooling Cost Model}

==> tables/number_of_metal_layer.tex <==
\begin{table}[]
\caption{Numbers of metal layers under different technology nodes for different chip scales. Parameters: % where% the parameters are set as follows:
The Rent's exponent $p=0.6$, the number of gate modules $N_g=(\textrm{\# of Transistors})/(4 \textrm{ Million})$, the fanout $f.o.=4$, the wire pitch $w=3.6\lambda$, the utilization efficiency of metal layers $\eta=0.1$.}\vspace{-5pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}TechNode\\  $\lambda$\ (nm)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tx Density\\ (MTx/mm$^2$)\end{tabular}} & \multicolumn{6}{c|}{\# of Transistors} \\ \cline{3-8} 
                                                                          &                                                                                    & 1M & 10M & 100M & 1B & 10B & 100B \\ \hline
28                                                                        & 2.93                                                                               & 2  & 4   & 8    & 13 & 19  & 27   \\ \hline
20                                                                        & 4.89                                                                               & 2  & 4   & 7    & 12 & 18  & 25   \\ \hline
16                                                                        & 6.86                                                                               & 2  & 4   & 7    & 11 & 17  & 24   \\ \hline
12                                                                        & 10.63                                                                              & 1  & 4   & 7    & 10 & 16  & 22   \\ \hline
10                                                                        & 14.02                                                                              & 1  & 4   & 6    & 10 & 15  & 22   \\ \hline
7                                                                         & 24.11                                                                              & 1  & 3   & 6    & 9  & 14  & 20   \\ \hline
5                                                                         & 42.83                                                                              & 1  & 3   & 6    & 9  & 13  & 19   \\ \hline
\end{tabular}
}
\vspace{-10pt}
\label{tab:num_of_metal_layer}
\end{table}
